A Theoretical Study of Neural Network Expressive Power via Manifold Topology

A prevalent assumption regarding real-world data is that it lies on or close to a low-dimensional manifold. When deploying a neural network on data manifolds, the required size, i.e., the number of neurons of the network, heavily depends on the intricacy of the underlying latent manifold. While significant advancements have been made in understanding the geometric attributes of manifolds, it's essential to recognize that topology, too, is a fundamental characteristic of manifolds. In this study, we investigate network expressive power in terms of the latent data manifold. Integrating both topological and geometric facets of the data manifold, we present a size upper bound of ReLU neural networks.

==> experiment.tex <==
\begin{figure}[ht]
\centering
%\hspace{13pt}
  \begin{subfigure}{0.3\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{figures/1-torus-line.pdf}
  \caption{Solid torus of genus 1.}
  \label{fig:torus1}
  \end{subfigure}
  \begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/2-torus-line.pdf}
  \caption{Solid torus of genus 2.}
  \label{fig:torus2}
  \end{subfigure}
  %\hspace{10pt}
  \begin{subfigure}{0.35\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/size_vs_g_square_5l_fitted.pdf}
  \caption{Relation between network size and $\beta^2$.}
  \label{fig:topocurve}
  \end{subfigure}
  
  \vspace{-0.1in}
  \caption{Validation of topological complexity. (a,b) are samples from two solid tori with different topological complexity. Samples from the negative class, which is not shown, are sampled uniformly from the background. (c) showcases the linear regression results between the network size and the square of topological complexity. A $5$-layer neural network with adaptive width is trained to fit tori of varying genus $g$. The width of the network is increased until the training accuracy exceeds 0.95.}
  \label{fig:topocomplex}
  \vspace{-0.1in}
\end{figure}

In this section, we present numerical results that showcase our topological bound \(O\left(\frac{d^2\beta^2}{\epsilon}\right)\) in fixed dimension. Even though this bound is derived through construction and serves as an upper limit, it is intriguing to discover that the bound is tight and can be readily observed in experimental settings. In practical scenarios, when training networks of varying sizes on data drawn from manifolds with different total Betti numbers \( \beta \), and achieving the same error rate, we anticipate a linear relationship between the network size and \( \beta^2 \).

We utilize manifolds characterized as solid genus-\(g\) tori, with \(g\) spanning from \(1\) to \(10\). Each genus-\(g\) torus is synthesized by overlapping two identical tori. For each torus, we consistently sample \(g\times10^4\) points from a surrounding bounding box. The labels for these points are generated using the indicator function of the solid torus. 

For training, we deploy a 5-layer ReLU network, gradually increasing its width until the training accuracy surpasses \(0.95\). Figure~\ref{fig:topocurve} presents a regression line charting the relationship between network size and the squared topological complexity, \(\beta^2\). This regression underscores a pronounced linear association between network size \(s\) and \(\beta^2\), with a correlation coefficient \(r = 0.9698\).



